Local and Global Decoding in Text Generation

Text generation, a key component in applications such as dialogue systems, relies on decoding algorithms that sample strings from a language model distribution. Traditional methods, such as top-$k$ and top-$\pi$, apply local normalisation to the model's output distribution, which can distort it. In this paper, we investigate the effect of this distortion by introducing globally-normalised versions of these decoding methods. Additionally, we propose an independent Metropolis-Hastings algorithm to approximate sampling from globally-normalised distributions without explicitly computing them. Our empirical analysis compares the performance of local and global normalisation across two decoding algorithms (top-$k$ and top-$\pi$) with various hyperparameters, using Pythia language models. Results show that, in most configurations, global decoding performs worse than the local decoding version of the same algorithms -- despite preserving the distribution's integrity. Our results suggest that distortion is an important feature of local decoding algorithms.

==> assets/table_samples.tex <==
\newcommand{\tablelinespacing}{7pt}
% \begin{table}[h]
\begin{table*}[h!]
    \centering
    \label{crouch}
    % \resizebox{.85\linewidth}{!}{%
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{  l  p{8cm}  p{8cm} }
        \toprule
% \textbf{Research Paradigm}      
& \multicolumn{1}{c}{\textbf{Local Decoding}}
& \multicolumn{1}{c}{\textbf{Global Decoding}} \\\midrule
$\alphabetkeeptopkwithval{|\alphabet|}$  
&        
\detokenize{
Xmas is exciting this year with the discovery of the new Dave.\n\nBelow you can see the new Dave in a 
}
& 
\detokenize{
Q:\n\nHow to start VLC using jars from android\n\nI am trying to start VLC using JPMS provided by Wizard
}
\\\midrule
$\alphabetkeeptopkwithval{5}$  
&        
\detokenize{
Q:\n\nHow to use the new.NET 4.0 framework with Mono 2.8.7 on Ubuntu 11.10?\n\nHow can I use the new.NET
}
& 
\detokenize{
\n#ifndef BOOST_MPL_AUX_TEMPLATE_ARIT
Y_HPP_INCLUDED\n#define BOOST_MPL_AUX_TEMPLATE_ARITY_HPP_IN
CLUDED
}
\\[\tablelinespacing]
$\alphabetkeeptopkwithval{10}$ 
&        
\detokenize{
\n\nI just read about the first time the UW football team beat Iowa, and I thought it was really cool:
}
& 
\detokenize{
1\n
}
\\[\tablelinespacing]
$\alphabetkeeptopkwithval{50}$  
&        
\detokenize{
Hurricane Dorian has left at least 15 dead and hundreds missing in the Bahamas as it approaches the
}
& 
\detokenize{
#ifndef OSQA_CONFIG_H_\n#define OSQA_CONFIG_H_\n\n/** @file\n *\n * Definitions shared by all platforms\n 
}
\\[\tablelinespacing]
$\alphabetkeeptopkwithval{100}$  
&        
\detokenize{
Tag: politics\n\nOn the afternoon of Wednesday, May 17th, I joined hundreds of thousands of other Amer
}
& 
\detokenize{
/*\nCopyright The Kubernetes Authors.\n\nLicensed under the Apache License, Version 2.0 (the "License")
}
\\[\tablelinespacing]
$\alphabetkeeptopkwithval{500}$  
&        
\detokenize{
Results of hyperthermic intraperitoneal chemotherapy versus hyperthermic intraperitoneal chemotherap
}
& 
\detokenize{
<?xml version="1.0" encoding="UTF-8"?>\n<!--  Copyright (C) 2013 The Android Open Source Project\n\n
}
\\[\tablelinespacing]
$\alphabetkeeptopkwithval{1000}$   
&        
\detokenize{
Peace love, Hope and Fasting.\n\nThursday, November 10, 2008\n\nOkay...A few weeks ago I had an interest
}
& 
\detokenize{
define("ace/mode/javascript_highlight_rules",["requ
ire","exports","module","ace/lib/oop","ace/mode/t
}
\\[\tablelinespacing]
$\alphabetkeeptopkwithval{5000}$  
&        
\detokenize{
West Lafayette\n\nIndiana’s unexpected first visit to baseball crowncases its home team’s success from
}
& 
\detokenize{
\n624 P.2d 352 (1981)\n105 Idaho 1002\nSue HANKS, Plaintiff-Appellant,\nv.\nHARTSDALE TOWNSHIP, Defendant
}
\\[\tablelinespacing]
$\alphabetkeeptopkwithval{10000}$
&        
\detokenize{
These algorithms have a "signature capture score"\nof about 3.\n
}
& 
\detokenize{
Beth Cooper\n\nNew York Times best-selling author Beth Cooper will deliver a lecture on poetry and cul
}
% \\[\tablelinespacing]
\\\midrule
$\alphabetkeeptoppwithval{0.01}$
&        
\detokenize{
Q:\n\nHow to get the value of a variable in a function?\n\nI have a function that is called from a butto
}
& 
\detokenize{
Q:\n\nHow to get the value of a variable in a function?\n\nI have a function that is called from a butto
}
\\[\tablelinespacing]
$\alphabetkeeptoppwithval{0.05}$
&        
\detokenize{
This invention relates to a semiconductor device and a method of manufacturing the same, and more pa
}
& 
\detokenize{
\n#include "qabstractnetworkmodel.h"\n
}
\\[\tablelinespacing]
$\alphabetkeeptoppwithval{0.25}$
&        
\detokenize{
The present invention relates to a semiconductor device and a method of manufacturing the same, and 
}
& 
\detokenize{
/*\n * Copyright (c) 2017-2018 THL A29 Limited, a Tencent company. All Rights Reserved.\n *\n * License
}
\\[\tablelinespacing]
$\alphabetkeeptoppwithval{0.5}$
&        
\detokenize{
K. T. P. S. B. P. C.\n\nK. T. P. S. B. P. C. is a small town in the Indian state of Uttar Pradesh. It 
}
& 
\detokenize{
import { IconDefinition, IconPrefix, IconName } from "@fortawesome/fontawesome-common-types";\nexport
}
\\[\tablelinespacing]
$\alphabetkeeptoppwithval{0.75}$
&        
\detokenize{
YAML 1.1\n\%TAG!u! tag:unity3d.com,2011:\n---!u!21 &2100000\nMaterial:\n  serializedVersion: 6\n  m_Objec
}
& 
\detokenize{
export { default as Slider } from './Slider';\n
}
\\[\tablelinespacing]
$\alphabetkeeptoppwithval{0.9}$
&        
\detokenize{
---\nabstract: 'We investigate the concept of the infinite divisibility of simple functions using som
}
& 
\detokenize{
Embodiments described herein relate to a device for testing nerve stimulation therapy for chronic pa
}
\\[\tablelinespacing]
$\alphabetkeeptopkwithval{0.95}$
&        
\detokenize{
Secretary of State Rex Tillerson, Defense Secretary Jim Mattis, CENTCOM Commander Army Gen. Lloyd Au
}
& 
\detokenize{
export * from './domain.module';\nexport { useLinkTo, registerLinkTo } from './utils';\n
}
\\[\tablelinespacing]
$\alphabetkeeptoppwithval{0.99}$
&        
\detokenize{
Associated Press\n\nSYRACUSE, N.Y. (AP) - A retired Northeastern University professor has been ordered
}
& 
\detokenize{
Along the dark, shadowy streets of ChicoMira moving south on Angioteque, cops have spotted three bro
}
\\
\bottomrule
\end{tabular}%
}
\caption{Texts generated with pythia-1.4b using local and global decoding. We present one randomly selected text for each configuration. The sequences are trimmed to 100 characters for readability.}
\label{tab:samples}
\end{table*}



% \begin{table*}[t]
%     \label{crouch}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{  l  p{8cm}  p{8cm} }
%         \toprule
% % \textbf{Research Paradigm}      
% & \multicolumn{1}{c}{\textbf{Local Normalization}}
% & \multicolumn{1}{c}{\textbf{Global Normalization}} \\\midrule
% $\alphabetkeeptopkwithval{|\alphabet|}$  
% &        
% \detokenize{
% Xmas is exciting this year with the discovery of the new Dave.\n\nBelow you can see the new Dave in a 
% }
% & 
% \detokenize{
% Q:\n\nHow to start VLC using jars from android\n\nI am trying to start VLC using JPMS provided by Wizard
% }
% \\[\tablelinespacing]
% $\alphabetkeeptopkwithval{5}$  
% &        
% \detokenize{
% Q:\n\nHow to use the new.NET 4.0 framework with Mono 2.8.7 on Ubuntu 11.10?\n\nHow can I use the new.NET
% }
% & 
% \detokenize{
% \n#ifndef BOOST_MPL_AUX_TEMPLATE_ARIT
% Y_HPP_INCLUDED\n#define BOOST_MPL_AUX_TEMPLATE_ARITY_HPP_IN
% CLUDED
% }
% \\[\tablelinespacing]
% $\alphabetkeeptopkwithval{10}$ 
% &        
% \detokenize{
% \n\nI just read about the first time the UW football team beat Iowa, and I thought it was really cool:
% }
% & 
% \detokenize{
% 1\n
% }
% \\[\tablelinespacing]
% $\alphabetkeeptopkwithval{50}$  
% &        
% \detokenize{
% Hurricane Dorian has left at least 15 dead and hundreds missing in the Bahamas as it approaches the
% }
% & 
% \detokenize{
% #ifndef OSQA_CONFIG_H_\n#define OSQA_CONFIG_H_\n\n/** @file\n *\n * Definitions shared by all platforms\n 
% }
% \\[\tablelinespacing]
% $\alphabetkeeptopkwithval{100}$  
% &        
% \detokenize{
% Tag: politics\n\nOn the afternoon of Wednesday, May 17th, I joined hundreds of thousands of other Amer
% }
% & 
% \detokenize{
% /*\nCopyright The Kubernetes Authors.\n\nLicensed under the Apache License, Version 2.0 (the "License")
% }
% \\[\tablelinespacing]
% $\alphabetkeeptopkwithval{500}$  
% &        
% \detokenize{
% Results of hyperthermic intraperitoneal chemotherapy versus hyperthermic intraperitoneal chemotherap
% }
% & 
% \detokenize{
% <?xml version="1.0" encoding="UTF-8"?>\n<!--  Copyright (C) 2013 The Android Open Source Project\n\n
% }
% \\[\tablelinespacing]
% $\alphabetkeeptopkwithval{1000}$   
% &        
% \detokenize{
% Peace love, Hope and Fasting.\n\nThursday, November 10, 2008\n\nOkay...A few weeks ago I had an interest
% }
% & 
% \detokenize{
% define("ace/mode/javascript_highlight_rules",["requ
% ire","exports","module","ace/lib/oop","ace/mode/t
% }
% \\[\tablelinespacing]
% $\alphabetkeeptopkwithval{5000}$  
% &        
% \detokenize{
% West Lafayette\n\nIndiana’s unexpected first visit to baseball crowncases its home team’s success from
% }
% & 
% \detokenize{
% \n624 P.2d 352 (1981)\n105 Idaho 1002\nSue HANKS, Plaintiff-Appellant,\nv.\nHARTSDALE TOWNSHIP, Defendant
% }
% \\[\tablelinespacing]
% $\alphabetkeeptopkwithval{10000}$
% &        
% \detokenize{
% These algorithms have a "signature capture score"\nof about 3.\n
% }
% & 
% \detokenize{
% Beth Cooper\n\nNew York Times best-selling author Beth Cooper will deliver a lecture on poetry and cul
% }
% \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Texts generated with pythia-410m using local normalisation and global normalisation. We present one randomly selected text for each configuration. The sequences are trimmed to 100 characters for readability.}
% \label{tab:samples}
% \end{table*}
